String Sound Synthesizer on GPU-accelerated Finite Difference Scheme

This paper introduces a nonlinear string sound synthesizer, based on a finite difference simulation of the dynamic behavior of strings under various excitations. The presented synthesizer features a versatile string simulation engine capable of stochastic parameterization, encompassing fundamental frequency modulation, stiffness, tension, frequency-dependent loss, and excitation control. This open-source physical model simulator not only benefits the audio signal processing community but also contributes to the burgeoning field of neural network-based audio synthesis by serving as a novel dataset construction tool. Implemented in PyTorch, this synthesizer offers flexibility, facilitating both CPU and GPU utilization, thereby enhancing its applicability as a simulator. GPU utilization expedites computation by parallelizing operations across spatial and batch dimensions, further enhancing its utility as a data generator.

==> fig/modal.tex <==
\begin{figure}[t]
    \begin{minipage}[b]{0.5\linewidth}
        \centering
        \centerline{\includegraphics[width=1.08\linewidth]{src/mode-rainbow.png}}
        \vspace{-2mm}
        \centerline{(a) Rainbowgram}
    \end{minipage}
    \begin{minipage}[b]{0.5\linewidth}
        \centering
        \centerline{\includegraphics[width=0.9\linewidth]{src/mode-f0.png}}
        \vspace{-2mm}
        \centerline{(b) $f_0$}
    \end{minipage}
    \label{fig: modal}
    \vspace{-2mm}
    \caption{Caption}
\end{figure}

